Visible but Not Yet Curatable: Characterizing the Curatability of Compact and Derived Open LLM Artifacts

Open Large Language Model (LLM) research increasingly produces compact and derived artifacts, such as adapters, quantized checkpoints, merged models, and distilled variants, that are distributed across papers, model hubs, model cards, code repositories, and release statements. Although these artifacts are publicly visible, digital libraries often lack sufficient evidence to identify, preserve, and cite them as coherent scholarly objects. We introduce a framework that conceptualizes curatability as a record-level property of distributed scholarly records and operationalizes it through four evidence dimensions: artifact identity, scholarly linkage, upstream evidence, and release assets. Guided by this framework, we conduct the first collection-scale characterization of open LLM curatability using a May 2026 snapshot of 191,375 public Hugging Face repositories and a core corpus of 2,214 scholarly papers. Our results reveal a pronounced visibility-to-curatability funnel. While 90.7% of paper records contain at least one useful curation signal, only 18.1% combine usable upstream evidence with concrete release evidence, and only 6.1% provide sufficiently coordinated evidence to support high-curatability records. Based on these findings, we derive a minimal seven-field curatable record and complementary responsibilities for model hubs, scholarly indexes, and digital libraries, providing practical guidance for improving the preservation and bibliographic control of open LLM artifacts.

==> tables/table_study_design.tex <==
\begin{table*}[!tbp]
\centering
\caption{Measurement constructs and checks. Each row maps one curation construct to its denominator, signal, calibration check, and supported claim.}
\label{tab:measurement-constructs}
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{0.98\textwidth}{@{}p{0.16\textwidth}p{0.17\textwidth}Yp{0.17\textwidth}p{0.17\textwidth}@{}}
\toprule
\tableheader
\textbf{Construct} & \textbf{Unit} & \textbf{Signal} & \textbf{Check} & \textbf{Output claim} \\
\midrule
Artifact identity & 191,375 repos & Role + package form & 300-role audit & Typed identity \\
Scholarly linkage & Repos + 2,214 records & HF/GitHub links; backlinks & Alignment split & Typed relation \\
Provenance & 2,214 records & Upstream tier $P$ & 200-row audit & Upstream claim \\
Release package & 2,214 records & Release tier $R$ & 50-URL audit & Visible assets \\
\rowcolor{TableGreen}
\textbf{Integrated} & 2,214 records & \textbf{P/R/L rule} & Sensitivity & \textbf{Readiness status} \\
\bottomrule
\end{tabularx}
\renewcommand{\arraystretch}{1.0}
\end{table*}

